Physical, chemical and morphological evolution of incipient soot obtained from molecular dynamics simulation of acetylene pyrolysis

Incipient soot particles obtained from a series of reactive molecular dynamics simulations were studied to understand the evolution of physical, chemical, and morphological properties of incipient soot. Reactive molecular dynamics simulations of acetylene pyrolysis were performed using ReaxFF potential at 1350, 1500, 1650, and 1800 K. A total of 3324 incipient soot particles were extracted from the simulations at various stages of development. Features such as the number of carbon and hydrogen atoms, number of ring structures, mass, C/H ratio, radius of gyration, surface area, volume, atomic fractal dimension, and density were calculated for each particle. The calculated values of density and C/H ratio matched well with experimental values reported in the literature. Based on the calculated features, the particles were classified in two types: type 1 and type 2 particles. It was found that type 1 particles show significant morphological evolution while type 2 particles undergo chemical restructuring without any significant morphological change. The particle volume was found to be well-correlated with the number of carbon atoms in both type 1 and type 2 particle, whereas surface area was found to be correlated with the number of carbon atoms only for type 1 particles. A correlation matrix comparing the level of correlation between any two features for both type 1 and type 2 particle was created. Finally, based on the calculated statistics, a set of correlations among various physical and morphological parameters of incipient soot was proposed.

==> preamble.tex <==
%\usepackage{epstopdf}% To incorporate .eps illustrations using PDFLaTeX, etc.
%\usepackage[caption=false]{subfig}% Support for small, `sub' figures and tables
%\usepackage[nolists,tablesfirst]{endfloat}% To `separate' figures and tables from text if required

%\usepackage[doublespacing]{setspace}% To produce a `double spaced' document if required
%\setlength\parindent{24pt}% To increase paragraph indentation when line spacing is doubled
%\setlength\bibindent{2em}% To increase hanging indent in bibliography when line spacing is doubled

%%%%%%%%%%%%%%%%%%%% Bibtex set up %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage[numbers,sort&compress]{natbib}% Citation support using natbib.sty
%\bibpunct[, ]{[}{]}{,}{n}{,}{,}% Citation support using natbib.sty
%\renewcommand\bibfont{\fontsize{10}{12}\selectfont}% Bibliography support using natbib.sty

%%%%%%%%%%%%%%%%%% Theore and Lemma etc. %%%%%%%%%%%%%%%%%%%%%
%\theoremstyle{plain}% Theorem-like structures provided by amsthm.sty
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}

%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{example}[theorem]{Example}

%\theoremstyle{remark}
%\newtheorem{remark}{Remark}
%\newtheorem{notation}{Notation}

%% This list environment is used for the references in the
%% Program Summary
%%
\newcounter{bla}
\newenvironment{refnummer}{%
   \list{[\arabic{bla}]}%
   {\usecounter{bla}%
      \setlength{\itemindent}{0pt}%
      \setlength{\topsep}{0pt}%
      \setlength{\itemsep}{0pt}%
      \setlength{\labelsep}{2pt}%
      \setlength{\listparindent}{0pt}%
      \settowidth{\labelwidth}{[9]}%
      \setlength{\leftmargin}{\labelwidth}%
      \addtolength{\leftmargin}{\labelsep}%
      \setlength{\rightmargin}{0pt}}}
{\endlist}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Others %%%%%%%%%%%%%%%%%%%%
%my own adjustments
\usepackage{lineno}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage[table,xcdraw]{xcolor}
%\usepackage{graphics}
%\usepackage{xkeyval}
% \usepackage{subfigure}
% \usepackage{subcaption}
\usepackage{subfig}
%\usepackage[graphicx]{realboxes}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{layout}
%\usepackage{multirow}
\usepackage{gensymb}
\usepackage{listings}

\lstset{
   breaklines=true,
   basicstyle=\ttfamily}

\usepackage{comment}
\usepackage{verbatim}
%\usepackage{verbatimbox}
%\usepackage{caption}
% \usepackage{subcaption}
%\captionsetup{compatibility=false}

%\usepackage{float}
%\usepackage{titlesec}
%\usepackage{pdflscape}
%\usepackage{adjustbox}
%\usepackage{rotating}
\usepackage{hyperref}
%\usepackage[figuresleft]{rotating}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
%\usepackage{textcomp}
%\usepackage{gensymb}

%\usepackage[tablesfirst,nomarkers,nolists]{endfloat}
%\DeclareDelayedFloatFlavor{sidewaystable}{table}
%\DeclareDelayedFloatFlavor{sidewaysfigure}{figure}
\usepackage{fancyvrb}
\usepackage[normalem]{ulem} %for strikethrough
\usepackage{enumitem}
% \renewcommand{\labelitemi}{$\circ$}
\renewcommand{\labelitemii}{$\circ$}
\renewcommand{\labelitemiii}{\tiny$\blacksquare$}
\renewcommand{\labelitemiv}{\tiny$\square$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Figure Location %%%%%%%%%%%%%%%%%

% \usepackage{multirow}
% \usepackage{graphicx}
% \graphicspath{{figures/}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Line Numbers %%%%%%%%%%%%%%%%%%

%\usepackage[modulo]{lineno}
%\linenumbers

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Random Text %%%%%%%%%%%%%%%%%%
%\usepackage{blindtext}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Version Control %%%%%%%%%%%%%%%%
\usepackage[table,xcdraw]{xcolor}
